Learning to Generalize to Unseen Tasks with Bilevel Optimization

Recent metric-based meta-learning approaches, which learn a metric space that generalizes well over combinatorial number of different classification tasks sampled from a task distribution, have been shown to be effective for few-shot classification tasks of unseen classes. They are often trained with episodic training where they iteratively train a common metric space that reduces distance between the class representatives and instances belonging to each class, over large number of episodes with random classes. However, this training is limited in that while the main target is the generalization to the classification of unseen classes during training, there is no explicit consideration of generalization during meta-training phase. To tackle this issue, we propose a simple yet effective meta-learning framework for metricbased approaches, which we refer to as learning to generalize (L2G), that explicitly constrains the learning on a sampled classification task to reduce the classification error on a randomly sampled unseen classification task with a bilevel optimization scheme. This explicit learning aimed toward generalization allows the model to obtain a metric that separates well between unseen classes. We validate our L2G framework on mini-ImageNet and tiered-ImageNet datasets with two base meta-learning few-shot classification models, Prototypical Networks and Relation Networks. The results show that L2G significantly improves the performance of the two methods over episodic training. Further visualization shows that L2G obtains a metric space that clusters and separates unseen classes well.

==> approach.tex <==
\section{Approach}
%\begin{figure*}[t]
%	\centering
%	\hfill
%	\includegraphics[height=4cm]{figure/concept-2.pdf}\label{fig:context}
%	\hfill
%	\vspace{-0.1in}
%	\caption{\small \textbf{Our meta-learning framework.} A neural network takes as an input each class prototype set, and map it to a Gaussian distribution with mean and variance. KL divergences between sampled and context classes, and within context classes are maximized to learn to generalize on unseen classes.}
%	\vspace{-0.1in}
%\end{figure*}

\subsection{Problem Setting}
We start by introducing the general problem statement of meta-learning few-shot classification.
Since few-shot learning problems involve a low-data challenge, many existing works~\cite{vinyals2016matching,santoro2016meta,rezende2016one,snell2017prototypical} resort to meta-learning, which trains the model to generalize over a task distribution $p(\mathcal{T})$. This is done by training it over large number of episodes, where at each episode we train the model on a randomly sampled task $\mathcal{T}_t\sim p(\mathcal{T})$. 

 Each task consists of a support set $\S^\ts=\{S_c^\ts\}_{c=1}^C$ and a query set $\Q^\ts=\{Q_c^\ts\}_{c=1}^C$, where $S_c$ and $Q_c$ suppose the set of classes observed at meta-training and that for meta-testing time are exclusive. We assume that  $K$ sample examples are given from each $N$ classes, we call this setting as $N$-way $K$-shot problems. Our goal is to minimize the classification error for $N$-way $K$-shot problems sampled from the test dataset. 

In each episode, we build a few-shot learning problem by sampling data from training dataset and learn a classifier to solve any few-shot learning problem well through a large number of episodes. 
Formally, at meta-training time, for each task $\mathcal{T}_t$, $N$ classes are randomly choosen from the training dataset. Then for each class $c$, we randomly sample the support set $S_c^\ts = \{(\bx_j, y_j)\}_{j=1}^K$ and the query set $Q_c^\ts = \{(\bx_j, y_j)\}_{j=1}^q$ which $\bx_j$ is a example and $y_j$ is corresponding label. With $\S^\ts = \{S_c^\ts \}_{c=1}^C $ and $\Q^\ts = \{Q_c^\ts \}_{c=1}^C $, an task $\mathcal{T}_t$ is then defined as a tuple $(\S^\ts, \Q^\ts)$. This configuration of support set and query set is to mimic testing. In testing phase, we have support set and test set and perform a classification for test examples by referring support set. 

\subsection{Embedding-based Meta-learning for Few-shot Classification}
We briefly describe existing few-shot learning methods that meta-learns metric space~\cite{snell2017prototypical, yang2018learning, vinyals2016matching}. The goal of metric learning approaches is to obtain the optimal embedding function $f_\theta: \mathbb{R}^D \rightarrow \mathbb{R}^M$ with parameters $\theta$ for the given series of random splits of $\S^\ts$ and $\Q^\ts$. While using diverse forms of learning objective is possible depending on modeling assumption, for now we simply denote it as a $\loss$. For a new task $\mathcal{T}_t$, the metric learning apporaches encode each support instances $\bx \in S_c^\ts$ and query instances $\bx \in Q_c^\ts$ with the embedding function $f_\theta (\bx)$. Then, prototypes $\bc_i$ are constructed by adding or averaging embedding vectors of sample instances to represent each class:
\begin{align}
\bc_c = g(\{f_\theta(\bx): for\ all\ \bx \in S_^\ts\})
\end{align}
where $g$ is function to generate prototypes by taking embedding vectors of sample instances.
We can construct loss $\loss$ by computing distances between a query instance $f_\theta(\bx)$ and a set of prototypes $\{\bc_i\}$ for all class within the episode. The distance between the query and the prototype belonging to the same class is closer, otherwise the distance is getting far. Distance measure can be a fixed measure  $d$ such as Euclidean distance of ~\cite{snell2017prototypical} or be learned like $d_\phi$ with parameters $\phi$ such as ~\cite{yang2018learning}:
\begin{align}
\loss \leftarrow \{d_\phi(\bc_i, f_\theta (\bx)): for\ all\ i,\ \bx \in \Q  \}    
\end{align}

\subsection{Learning to Generalize to Unseen Classes}
Existing embedding-based approaches have learned metric space well for each given episode, which a classifier concentrates to sampled classes to assign query instances correctly. However, in this episodic training strategy, we always train the embedding function to classify only the sampled classes, even though there are actually more unseen classes in the common metric space. In this process, the embedding function tends to focus on optimizing the specific metric space for individual episodes rather than learning the generalized meta-knowledge to embed any unseen classes well into the metric space. Therefore we propose a framework that forces a model to explicitly learn transferrable meta-knowledge applicable to any episode. Specifically, we pair two episodes as one training unit and train the embedding function by learning of classification in one episode to be helpful to a classification of other episode in the training. The intuition behind this approach is that the network learn transferrable internal features to classify explicitly rather than episode-specific features.  

For this, we adopt gradient-based update strategy of MAML~\cite{finn2017model}. Parameters of network is updated with gradients which generated from a loss of the first episode and the learned network perform a classification of the second episode. While the goal of MAML~\cite{finn2017model} is to learn good initial parameters and requires a fine-tuning with several gradient steps to adapt fast to new task, the goal of our model is to learn generalized embedding parameters for unseen classes. In meta-test phase, we test our model only with initial parameters. As show in table ~\ref{tbl:mini} and \ref{tbl:tiered}, without fine-tuning, our model outperforms baselines since initial parameters already learn generic embedding. 

Formally, we update parameters $\theta, \phi$ with gradient descents computed from $\loss$:
\begin{align}
\{\theta', \phi' \} \leftarrow \{\theta, \phi \} - \alpha \nabla_{\{\theta, \phi\}} \loss_{\EE_1}(f_\theta, d_\phi) 
\end{align}

In our case, the step size $\alpha$ is fixed hyperparameter but, we can change it to be learnable such as Meta-SGD~\cite{li2017meta}. We sample a second episode $\EE_2$ that classes are disjoint with classes of episode $\EE_i$ and compute a loss $\loss_{\EE_j}(f_{\theta'}, d_{\phi'})$ with updated parameters $\theta', \phi'$ by encoding query input and prototypes of $\EE_j$ and computing distance between each class and corresponding query instances. Then our meta-objective is defined as:

\begin{align}
min_{\theta, \phi} {\loss_{\EE_2}}(f_{\theta'}, d_{\phi'}) = {\loss_{\EE_2}(f_{\theta-\alpha \nabla_{\theta} \loss_{\EE_1}(f_\theta, d_\phi)}, d_{\phi-\alpha \nabla_{\phi} \loss_{\EE_1}(f_\theta, d_\phi)})}
\end{align}

Note that when the model parameters are updated using the gradients computed from the first episode, the model parameters are optimized to perform the classfication of the second episode. It means that the model learn effective generalized classification for unseen classes across episodes. The meta-update is performed as follows:
\begin{align}
\{\theta, \phi\} \leftarrow \{\theta, \phi\} - \beta \nabla_{\{\theta, \phi\}} \loss_{\EE_2}(f_{\theta'}, d_{\phi'})
\end{align}

$\beta$ is the meta step size. 

\begin{algorithm}[t]
	\caption{Learning to Genearalize to Unseen Tasks}\label{algo:L2G}
	\begin{algorithmic}[1]
		\State $\alpha, \beta$: step size hyperparameters
		\For{each \emph{iteration}}
		\State Sample batch of tasks
		\For{each \emph{task t}}
		\State Sample the first episode $\EE^{ t }_1 = (\S, \Q)$
		\State Compute the loss for each query instances $\bx \in \Q$ with $\{\bc_i \}$ using $f_\theta$ and $d_\phi$:
		\State $\loss \leftarrow \{d_\phi(\bc_i, f_\theta (\bx)): for\ all\ i,\ \bx \in \Q  \}$    
		\State Evaluate $\nabla_{\{\theta, \phi\}} \loss_{\EE^{ (t) }_1}(f_\theta, d_\phi)$  in Equation (2)
		\State Compute adapted parameters with gradient descent:
		\State $\{\theta', \phi' \} \leftarrow \{\theta, \phi \} - \alpha \nabla_{\{\theta, \phi\}} \loss_{\EE^{(t)}_1}(f_\theta, d_\phi) $
		\State Sample the second episode $\EE^{ (t) }_2 = (\S, \Q)$ for meta-update
		\EndFor
		\State Update $\{\theta, \phi\} \leftarrow \{\theta, \phi\} - \beta \nabla_{\{\theta, \phi\}} \sum_t \loss_{\EE^{ (t) }_2}(f_{\theta'}, d_{\phi'})$ using $\mathcal{L}_{\EE^{ (t) }_2}$ in Equation (4)
		\EndFor
	\end{algorithmic}
\end{algorithm}


\subsection{Application to Metric-Based Methods}
We apply the proposed framework to two representative embedding-based methods. To show that our proposed framework works for any metric-space based model generally, we combine the proposed framework with two representative metric-space based baselines: 1. Our framework + Prototypical Network (Ours + Proto). 2. Our framework + Relation Network (Ours + RN). In the meta-training process, both versions sample two episodes and train a network to learn a generic embedding method by forcing the way learned in one episode to be helpful to perform classification on the other episode.
\paragraph{Prototypical Networks~\cite{snell2017prototypical}}
This is an embedding-based model that uses the embedding of the sample mean as the class prototype. The model is discriminatively trained to minimize the relative Euclidean distance between each instance and its correct class embedding to other class embeddings. Each prototype is a mean vector of sample features of each class.
\begin{align}
\bc_i = \frac{1}{|S_i|}\sum_{\bx \in S_i} f_\theta(\bx)
\end{align}
Distance measure is Euclidean distance:
\begin{align}
d(\bc_i, f_\theta(\bx_j)) = ||\bc_i - f_\theta(\bx_j)||^2
\end{align}
Ojective function $\loss$ is (based on a softmax over distances to the prototypes in the embedding space)(with the negative log-probability):
\begin{equation}
\begin{aligned}
&\loss_{\theta} = \sum_{i}^N \left[ \sum_{\bx \in Q_i} \left[ d\Big(\bc_i, f_\theta(\bx)\Big) + \log \sum_{j}^N \exp\Big(-d\Big(\bc_j, f_\theta(\bx\Big)\Big)\right] \right] \label{eq:disc_loss}
\end{aligned}
\end{equation}

\paragraph{Relation Net~\cite{yang2018learning}}
This is a model that learns a distance metric by stacking multiple layers with nonlinearity, on the concatenated vectors for each class prototype and query instance to generate relation scores between them. An embedding function $f_\theta$ of Relation Net produces features $f_\theta(\bx)$ of query instances and sample instances of each class. Relation Net creates prototypes $c_i$ by adding features from sample instances of each class. 
\begin{align}
\bc_i = \sum_{\bx \in S_i} f_\theta(\bx)
\end{align}
Each prototype  and query instances are concatenated. Relation module which are learnable distance measure are used to compute relation scores between each query instance $\bx_j$ and prototypes of classes:
\begin{align}
s_{i,j} = d_\phi(concat(\bc_i, f_\theta(\bx_j)))
\end{align}
Relation Net uses mean square error (MSE) as the objective function:
\begin{align}
\loss_{\theta, \phi} = \sum_i^m\sum_j^n(s_{i,j} - 1)_{i=j}^2 + (s_{i,j})^2_{i \neq j}
\end{align}
The model is trained so that relation scores of matched a query, prototype combination is 1 and those of not matched pair is 0. 




%\begin{figure*}[t]
%	\centering
%	\includegraphics[height=3.2cm]{figure/loss_context.pdf}\label{loss_context}
%	\vspace{-0.1in}
%	\caption{\small dsdd
%	}
%	\vspace{-0.1in}
%\end{figure*}

==> approach_backup_2.tex <==
\section{Approach}
\label{approach}
%\begin{figure*}[t]
%	\centering
%	\hfill
%	\includegraphics[height=4cm]{figure/concept-2.pdf}\label{fig:context}
%	\hfill
%	\vspace{-0.1in}
%	\caption{\small \textbf{Our meta-learning framework.} A neural network takes as an input each class prototype set, and map it to a Gaussian distribution with mean and variance. KL divergences between sampled and context classes, and within context classes are maximized to learn to generalize on unseen classes.}
%	\vspace{-0.1in}
%\end{figure*}

\subsection{Problem Definition}
We start by describing the episodic training which firstly introduced in ~\cite{vinyals2016matching}
We introduce the general problem statement of few-shot learning. We start by dividing the given dataset into mutual exclusive training and test sets. When $N$ sample examples are given from each $C$ classes, we call this setting as $C$-way $N$-shot problems. Our goal is to minimize the classification error for $C$-way $N$-shot problems sampled from the test dataset. Since few-shot learning problems have a low-data challenge, many existing works~\cite{vinyals2016matching,santoro2016meta,rezende2016one,snell2017prototypical} resort to meta-learning, which trains the model to generalize over a task distribution $p(\mathcal{T})$. This is done by training it over large number of episodes, where at each episode we train the model on a randomly sampled few-shot classification task $\mathcal{T}_t\sim p(\mathcal{T})$. By training over large number of randomly sampled few-shot classification tasks, $\mathcal{T}_1, \dots, \mathcal{T}_T$, we expect to obtain generic knowledge for classification that can be utilized to solve any few-shot learning problems at the meta-test time.

Formally, at meta-training time, for each episode $t$, the task $\mathcal{T}_t$ consists of $C$ classes are randomly selected from the training dataset. Then for each class $c$, we randomly sample the support set $S_c = \{\bx_{c, n}\}_{n=1}^N$ and the query set $Q_c = \{\tilde{\bx}_{c, m}\}_{m=1}^M$. By aggregating the support and the query set for all classes as $\S = \{S_c \}_{c=1}^C $ and $\Q = \{Q_c \}_{c=1}^C $, we can define an task $\EE$ is as a tuple $(\S, \Q)$. At meta test time, we are given a task $\mathcal{T}_{test} = (\S_{test}, \Q_{test})$ where $\S_{test}$ and $\Q_{test}$ contain examples of classes unseen during meta-training time. 

\subsection{Embedding-based Few-shot Learning Apporaches}
We briefly describe a generic framework for metric-based few-shot meta-learning methods~\cite{snell2017prototypical, yang2018learning, vinyals2016matching}. The goal of metric learning approaches is to obtain the optimal embedding function $f_\theta$ with parameters $\theta$ for the given series of task $\EE_1,\dots,\EE_T$. While using diverse forms of learning objective is possible depending on modeling assumption, for now we simply denote it as a $\loss$. For a given task $\EE_t$, the metric learning apporaches encode each support instance $\bx \in S_c$ and query instance $\tilde{\bx} \in Q_c$ with the embedding function $f_\theta$ for all $c$. Then, the prototype $\rho_c$ for class $c$ is constructed by adding or averaging embedding vectors to represent each class:
\begin{align}
\rho_c = g(\{f_\theta(\bx_{c,1}),\dots,f_\theta(\bx_{c,N})\})
\end{align}
where $g$ is function which generate a prototype from the embedding vectors of the sample instances.
We can construct loss $\loss$ by computing distance between a query instance $f_\theta(\bx)$ and a set of prototypes $\{\rho_c\}$ for all class within the given task. The distance measure $d(\cdot,\cdot)$ could either be a fixed measure, as with Prototypical Networks~\cite{snell2017prototypical} which leverage the Euclidean distance, or could be learned as with Relation Networks~\cite{yang2018learning} that trains the similarity measure between the two instances using a separate network with additional parameters. Then for a given task $\EE_t$ consisting of the support and query set, we minimize the following loss for all query examples $\tilde{\bx}$:
\begin{align}
\loss_{\EE_t}(\{\rho_c\}, f_\theta(\tilde{\bx})))
\end{align}
The loss should be minimized if $d(\rho_c, f_\theta(\tilde{\bx_c}))$, the distance between $\bx_c$ and its correct class prototype $\rho_c$, is minimized and $d(\rho_i, f_\theta(\tilde{\bx_c}))$ is large, where $i\ne{c}$. %Then we sum up all the losses to perform gradient descent w.r.t. $\theta$ and $\phi$.

\subsection{Learning to Generalize to Unseen Classes}
Existing embedding-based approaches learn a metric space over large number of episodes, where given a single episode, a classifier tries to correctly classify query instances based on the class prototypes. However, the main limitation of such an approach is that the embedding function is only trained for classifying given small set of classes at a time, which does not consider generalization of the learned embedding to unseen classes. This explains the reason the metric-based methods such as Prototypical Networks converge fast, but at the same time, trained embedding function may be suboptimal with its myopic optimization process.

To overcome this shortcoming, we propose a framework which enforces a model to \emph{explicitly} learn transferrable meta-knowledge applicable to any tasks. Specifically, we pair two tasks as a single training unit at each iteration, and train the embedding function by constraining the learning in one task to be helpful to another task during meta-training. The intuition behind this approach is that the network learns more generalizable and transferrable internal features rather than task-specific features.  

Toward this goal, we adopt a bilevel optimization framework that is similar to MAML~\cite{finn2017model}. The goal of MAML~\cite{finn2017model} is to learn most amenable initialization parameters and to reach specific parameters adapted to the given task through gradient-based parameter updates with this bilevel optimization framework. However, our goal is to learn generalizable parameters for unseen tasks by regularizing the first task which considers the task loss on the second task when it performs optimization. Therefore, different with MAML~\cite{finn2017model}, in the meta-testing time, our model solves the few-shot classification problems with generalized initial parameters, which do not need fine-tuning with gradient update for the given tasks. 

This is made possible by having the first task $\EE_i$ in the inner loop and the second task $\EE_j$ in the outer optimization loop, such that we update the shared network parameters for the second task with the gradients generated from the loss of the first task. Since learning on the task $\EE_i$ is regularized to work well for the task $\EE_j$, this will allow task $\EE_i$ to learn a transferrable generic knowledge useful for few-shot classification of any given set of classes. In Table ~\ref{tbl:mini} and \ref{tbl:tiered}, we show that our model outperforms baselines without finetuning since initial parameter is already optimized to minimize classification error on a task consisting of unseen classes. 

Formally, we construct an inner-gradient update step with the model parameters $\theta$:
\begin{align}
\theta' = \theta - \alpha \nabla_{\theta} \loss_{\EE_i}(\{\rho_c\}, f_\theta(\tilde{\bx})) 
\end{align}

In our case, the step size $\alpha$ is a fixed hyperparameter, but we can learn it as done with Meta-SGD~\cite{li2017meta}. We sample the second task $\EE_j$ from a \emph{disjoint} set of classes to the classes in the task $\EE_i$, and compute the loss $\loss_{\EE_j}(\{\rho_c\}, f_{\theta'}(\tilde{\bx}))$ with updated parameters $\theta'$ by encoding all query input and prototypes of $\EE_j$. Then our goal is to meta-learn a $\theta$ that minimizes the following meta-objective:

\begin{align}
\min_{\theta} {\loss_{\EE_j}}(\{\rho_c\}, f_{\theta'}(\tilde{\bx})) = {\loss_{\EE_j}(\{\rho_c\}, f_{\theta-\alpha \nabla_{\theta} \loss_{\EE_i}(\{\rho_c\}, f_\theta(\tilde{\bx}))}(\tilde{\bx}))}
\end{align}

Note that when the model parameters are updated using the gradients computed from the first task $\EE_i$, the model parameters are optimized to perform the classfication of the second task $\EE_j$. This allows the model to effectively learn the generalized classification for unseen classes across episodes. Then we can perform the meta-update as follows:
\begin{align}
\theta = \theta - \beta \nabla_{\theta} {\loss_{\EE_j}}(\{\rho_c\}, f_{\theta'}(\tilde{\bx}))
\end{align}

where $\beta$ is the meta step size. Algorithm 1 describes the detailed steps of our meta-learning algorithm.

\begin{algorithm}[t]
	\caption{Learning to Genearalize to Unseen Tasks}\label{algo:L2G}
	\begin{algorithmic}[1]
		\State $\alpha, \beta$: step size hyperparameters
		\For{each \emph{batch}}
			\For{each \emph{iteration}}
				\State Sample the first task $\EE_i = (\S, \Q)$
				\State Compute the inner gradient loss $\loss_{\EE_i}(\{\rho_c\}, f_\theta(\tilde{\bx})))$ for $\tilde{\bx} \in \Q$ with $\{\rho_c \}$ 
				%\State Compute the inner gradient loss for $\tilde{\bx} \in \Q$ with $\{\rho_c \}$ using $f_\theta$ and $d$:
				\State Evaluate $\loss_{\EE_i}(\{\rho_c\}, f_\theta(\tilde{\bx}))$  in Equation (2)
				\State Update the parameters with gradient descent:
				\State $\theta' = \theta - \alpha \nabla_{\theta} \loss_{\EE_i} $
				\State Sample the second task $\EE_j = (\S, \Q)$ for meta-update
			\EndFor
				\State {\color{red} $\theta = \theta - \beta \nabla_{\theta} {\loss_{\EE_j}}$ using ${\loss_{\EE_j}}(\{\rho_c\}, f_{\theta'}(\tilde{\bx}))$ in Equation (4)}
		\EndFor
	\end{algorithmic}
\end{algorithm}

\subsection{Learning to Generalize with Embedding-based Meta-Learners}
Our learning framework requires that the same model parameter could be used to solve two different tasks. While our algorithm is very simlar to MAML's algorithm except that we have two different tasks at the inner and the outer loop of the optimization framework, it is not compatible with MAML since the parameters of the softmax classifier for a few-shot classification task will not work for another few-shot classification task with different sets of classes. On the other hand, for metric-based models, a learned metric for one task is readily generalizable to another task without any modification, as it is essentially a task-generic space where we could embed any instances from any classes onto. 

While our method could work with any metric-based meta-learning methods, we apply the proposed framework to two most popular models, namely Prototypical Networks~\cite{snell2017prototypical} and Relation Networks~\cite{yang2018learning}.

\paragraph{Prototypical Networks~\cite{snell2017prototypical}}
This is a metric-based few-shot meta-learning model which is discriminatively trained to minimize the relative Euclidean distance between each instance and its correct class prototype over its distance to other class embeddings. Each prototype $\rho_c$ is a mean vector of the support instance embeddings $f_\theta(\bx)$:
\begin{align}
\rho_c = \frac{1}{|S_c|}\sum_{\bx \in S_c} f_\theta(\bx)
\end{align}
For distance measure, we use Euclidean distance:
\begin{align}
d(\rho_c, f_\theta(\tilde{\bx})) = ||\rho_c - f_\theta(\tilde{\bx})||^2
\end{align}
Objective function $\loss$ is based on a softmax over distances to the prototypes in the embedding space with the negative log-probability :
\begin{equation}
\begin{aligned}
&\loss_{\theta} = \sum_{c=1}^C \left[ \sum_{\tilde{\bx} \in Q_c} \left[ d\Big(\rho_c, f_\theta(\tilde{\bx})\Big) + \log \sum_{c'=1}^C \exp\Big(-d\Big(\rho_{c'}, f_\theta(\tilde{\bx})\Big)\Big)\right] \right] \label{eq:disc_loss}
\end{aligned}
\end{equation}

\paragraph{Relation Networks~\cite{yang2018learning}}
This model learns a distance metric using a subnetwork on the concatenated vectors of each class prototype and query instance to generate relation scores between them. An embedding function $f_\theta$ of a Relation Network produces features $f_\theta(\tilde{\bx})$ of query instances and sample instances $f_\theta(\bx)$ of each class. Relation Networks create prototypes $\rho_c$ by adding features from sample instances of each class. 
\begin{align}
\rho_c = \sum_{\bx \in S_c} f_\theta(\bx)
\end{align}
After concatenating each prototype and query instance, the relation module with learnable distance measure computes the relation score between each of the $m$ query instances and $c$ class prototypes:
\begin{align}
s_{c,m} = d(concat(\rho_c, f_\theta(\tilde{\bx}_m)))
\end{align}
Relation Net uses Mean Square Error (MSE) for the objective as follows:
\begin{align}
\loss_{\theta} = \sum_{n=1}^{N_t} \sum_{m=1}^{M_t}(s_{n,m} - 1)_{y_n=y_m}^2 + (s_{n,m})^2_{y_n \neq y_m}
\end{align}
where $N_t = C \times N, M_t = C \times M$ and $y$ denotes the labels. The model is trained to match the support and query instances in each class with the relation score that penalizes the incorrect predictions.
% 이게 제안된 방법과 어떻게 엮이는데??

%\paragraph{Application to MAML and other meta-learning approaches}
%Note that our learning to generalize framework is not compatible with MAML~\cite{finn2017model} although the algorithms for the two methods are only slightly different. This is because the parameter of the softmax classifier for one few-shot classification task will not work for another few-shot classification task with different sets of classes. Thus, without a mechanism to generate softmax classifier weight, it is not straightforwad to apply our L2G framework to MAML.

%In this section, we introduce our novel approach to solve the problem described above. Our goal is to learn embedding space from a set into a distribution in which embedded distributions corresponding to different classes are well separated. % to encode a set into a distribution, which also satisfies discriminativity between classes.
%Toward this, we devise a novel loss function $\loss$ that consists of two terms: (i) a generative loss to encode a set into a distribution and (ii) a discriminative loss to locate different distributions in separated regions.

%Our generative loss basically is built on similar intuition in   \cite{edwards2016towards}, with slight modification in the graphical structure (see below for details). The original Neural Statistician developed in \cite{edwards2016towards} assumes hierarchical latent variables to generate $\Dtr$: the first variable $\bc$ is to locate class-level variance, and the other variable $\bz$ captures instance-level variance \cite{kingma2014semi}. Each datapoint $\bx$ is assumed to be generated conditionally on those two latent variables. Unlike \cite{edwards2016towards}, we adopt the dependency between variables as shown in Figure \ref{model_gen} to simplify the inference procedure and allow efficient episodic meta-training\footnote{We also used this version of Neural Statistician as our baseline.}. For each episode, the generative process of the sampled dataset $\PP = \{\hat{\X}_1,\dots,\hat{\X}_S\}$ is as follows:
%\begin{align}
%p(\bc_i) = \N(\mathbf{0}, \bI),\quad p(\bz) = \N(\mathbf{0}, \bI),\quad p(\PP) = \prod_{i \in \mathcal{I}} \int p(\bc_i) \left[ \prod_{\bx \in \hat{\X}_i} \int p(\bz)p_\theta(\bx|\bz,\bc_i) \text{d}\bz \right] \text{d}\bc_i 
%\end{align}
%where $\theta$ is the collection of parameters for the generative process. Note that the exact posterior of $\bc$ and $\bz$ is intractable. Instead, we resort to variational mean-field approximation with tractable form of lower bound. If we further approximate it with a single Monte-Carlo sample, then we obtain the following generative loss:
%\begin{align}
%\loss_\text{gen}(\psi,\theta,\phi;\PP) = \sum_{i \in \mathcal{I}} \sum_{\bx \in \hat{\X}_i} \bigg(\log p_\theta(\bx|\tilde{\bc}_i,\tilde{\bz}) - \KL[q_\phi(\bz|\bx)\|p(\bz)]\bigg) - \KL[q_\psi(\bc_i|\hat{\X}_i)\|p(\bc_i)] \label{eq:gen_loss}
%\end{align}
%where $\tilde{\bc}_i$ and $\tilde{\bz}$ are sampled from $q_\psi(\bc_i|\hat{\X}_i)$ and $q_\phi(\bz|\bx)$ respectively, and backpropagated with reparameterization trick w.r.t. the variational parameters $\psi$ and $\phi$~\cite{kingma2013auto}. 

%\begin{figure*}[t]
%	\hfill
%	\subfigure[generative model]{\includegraphics[height=2.6cm]{figure/model-gen.pdf}\label{model_gen}}
%	\hfill
%	\subfigure[KL divergence for discriminating between classes]{\includegraphics[height=2.6cm]{figure/loss-disc.pdf}\label{loss_disc}}
%	\hfill
%	\vspace{-0.1in}
%	\caption{\small (a) The generative model for DiVaSE, for each sampled classes $i \in \mathcal{I}$ and dataset $\hat{\X}_i$. The posterior of $\bc_i$ is obtained given a dataset $\hat{\X}_i$, which is the embedding distribution we work with. (b) For all the class pairs $i,j \in \mathcal{I}$, the embedding of each query instance and the that of each support set are compared through KL divergence, to determine class identities of query instances.
%	}
%	%\vspace{-0.1in}
%\end{figure*}

%Note that $q_\psi$ is the embedding function discussed above, which maps set $\hat{\X}_i$ to the corresponding posterior distribution of $\bc_i$. In doing so, we use Deep set \cite{zaheer2017deep} to convert the set $\hat{\X}_i$ into a single vector, namely $\bv_i$. Specifically, each elements $\bx \in \hat{\X}_i$ is nonlinearly transformed with multiple layers denoted as $f_\psi(\bx)$ and they are collected and averaged into $\bv_i$. Finally, mean and log variance of $\bc_i$ are generated from $\bv_i$:
%\begin{align}
%	\bv_i = \frac{1}{\hat{N}_i} \sum_{\bx \in \hat{\X}_i} f_\psi(\bx),\quad q_\psi(\bc_i|\hat{\X}_i) = \N(\bs\mu_\psi(\bv_i),\text{diag}(\bs\sigma_\psi^2(\bv_i)))
%\end{align}
%In all our experiments, we use a single layer implementation for each $\bs\mu$ and $\bs\sigma$, which seems to perform better than applying additional nonlinearities on $\bv_i$.

%\subsection{Learning to Discriminate between Distributions}
%The most critical limitation of \cite{edwards2016towards} as a classifier is that the generative loss $\loss_\text{gen}$ embeds each class set independently. There is no explicit consideration for discriminating between embeddings for different classes, hence they start to collide and the performance degrades even with the moderate number of classes considered at a time. To solve this issue, we propose to minimize the distance $d(\cdot,\cdot)$ between the distribution of prototype set $q_\psi(\bc_i|\hat{\X}_i)$ and that of query instances $q_\psi(\bc_i|\bx), \bx \in (\X_i \backslash \hat{\X}_i)$ if they belong to the same class $i$. Otherwise, we maximize the distance between them:
%\begin{equation}
%\begin{aligned}
%&\loss_\text{disc}(\psi;\PP,\Q) \\
%&= \sum_{i \in \mathcal{I}} \left[ \sum_{\bx \in (\X_i \backslash \hat{\X}_i)}d\Big(q_\psi(\bc_i|\hat{\X}_i),q_\psi(\bc_i|\bx)\Big) + \log \sum_{j \in \mathcal{I}} \exp\Big(-d\Big(q_\psi(\bc_i|\hat{\X}_j),q_\psi(\bc_i|\bx)\Big)\Big)\right] \label{eq:disc_loss}
%\end{aligned}
%\end{equation}
%The form of the objective is log of softmax probabilities, which is similar to that of Prototypical Network~\cite{snell2017prototypical}. However, since we need to measure \emph{the similarity between two probabilistic distributions}, Euclidean distance or cosine similarity cannot be used as a proper metric. Here, although it is not a distance, we use Kullback-Leibler (KL) divergence, %such that for some probability distributions $P$ and $Q$,
%\begin{align}
%d(P,Q) := \KL[P\|Q].
%\end{align}
%While $\KL$ is not commutative, it turns out using opposite direction of KL divergence still works well mainly because both distributions in \eqref{eq:disc_loss} are in the same Gaussian family. 

%both direction Note that the direction of the divergence is from $Q$ to $P$.

%discriminative loss in \eqref{eq:disc_loss}. However, we still want to make our embedding function $q_\psi$ to consider even remaining classes (that is, classes not in $\I$) as well, which we call \emph{context classes}: $\C \subset [S]\backslash\I$. In order to achieve this purpose, we propose additional scheme where we periodically (e.g. for every 100th episode) store the set vector $\bv_i$ and use them to maximize the KL divergences even for context classes:    
%the classification within $\I$ also induce the discriminativity within $\C$, as well as between $\I$ and $\C$. Toward this goal, we maximize the KL divergences between the corresponding class pairs.%\footnote{Note that we arbitrarily set the direction of the KL divergence, they and can be changed.}
%\begin{align}
%\loss_\text{context}(\psi;\PP,\widebar{\mathcal{V}}) = %\underbrace{\sum_{i \in \mathcal{I}} \sum_{j \in \mathcal{C}} -d(q_\psi (\bc_i|\hat{\X}_i),q_\psi(\bc_j|\widebar{\bv}_j))}_\text{between sampled and context classes} + \underbrace{\sum_{i \in \mathcal{C}} \sum_{j \in \mathcal{C}} -d(q_\psi (\bc_i|\widebar{\bv}_i),q_\psi(\bc_j|\widebar{\bv}_j))}_\text{within context classes} \label{eq:context_loss}
%\end{align}
%where we abuse notation and $q_\psi (\bc_i|\widebar{\bv}_i) = \N(\bs\mu_\psi(\widebar{\bv}_i),\text{diag}(\bs\sigma_\psi^2(\widebar{\bv}_i)))$. This scheme is based on past embedding, which is not perfect, but can prevent severe collisions among unselected classes while greatly reducing the computational cost of inferring $q_\psi(\bc_i|\X_i)$ for all classes every episode.

%Here, $\widebar{\bv}_i$ is the set vector stored for each class $i \in [S]$, and we update them periodically with the predefined frequency (e.g. 100). It greatly reduces the computational cost of inferring $q_\psi(\bc_i|\X_i)$ every episode, because we do not have to forward pass $f_\psi(\bx)$ for all $\bx \in \X_i$. In this vein, $q_\psi(\bc_i|\widebar{\bv}_i)$ in \eqref{eq:context_loss} indicates that the posterior of $\bc_i$ can also be inferred from the pre-stored set vector $\widebar{\bv}_i$. The collection of $\widebar{\bv}_i$ for all $i \in [S]$ is denoted as $\widebar{\mathcal{V}}$.

%The final version of our learning algorithm is described in Algorithm \ref{algo:divase}. The model has two hyperparameters $\lambda$ and $\gamma$ for scaling each loss term. We can tune them via cross-validation in practice. More detailed experimental setup is introduced in the next section.




%\begin{figure*}[t]
%	\centering
%	\includegraphics[height=3.2cm]{figure/loss_context.pdf}\label{loss_context}
%	\vspace{-0.1in}
%	\caption{\small dsdd
%	}
%	\vspace{-0.1in}
%\end{figure*}

==> approach_new.tex <==
\section{Approach}
\begin{figure*}[t]
	\centering
	\hfill
	\includegraphics[height=4cm]{figure/concept-2.pdf}\label{fig:context}
	\hfill
	\vspace{-0.1in}
	\caption{\small \textbf{Our meta-learning framework.} A neural network takes as an input each class prototype set, and map it to a Gaussian distribution with mean and variance. KL divergences between sampled and context classes, and within context classes are maximized to learn to generalize on unseen classes.}
	\vspace{-0.1in}
\end{figure*}

We start by introducing the general problem statement. Define a set $[N] := \{1,\dots,N\}$. We consider the problem of generalizing to unseen classes, where we have a training set consisting of $S$ \emph{seen} classes: $\Dtr = \{\X_1,\dots,\X_S\}$, and a test dataset $\Dte = \{\X_{S+1},\dots,\X_{S+U}\}$ consisting of $U$ \emph{unseen} classes. Our goal then is to minimize the classification error between samples from this unseen classes. For each class $i \in [S+U]$, set $\X_i$ has $N_i$ number of datapoints $\bx_{i,1},\dots,\bx_{i,N_i}$. We do not assume that $N_i$ is fixed across classes, and in real-world datasets, $N_i$ may actually vary largely across classes. 

\paragraph{Episodes} At train time, we are interested in episodic distribution $\pepi$ where an episode is sampled from $\Dtr$. Specifically when generating an episode, a subset class indices $\mathcal{I} \subset [S]$ is first sampled, then for each class $i \in \mathcal{I}$, a subset $\hat{\X}_i \subset \X_i$ is sampled to form the prototype of the class. The collection of them is denoted as $\PP=\{\hat{\X}_i \subset \X_i: i \in \mathcal{I}\}$. The remaining instances in $\X_i \backslash \hat{\X}_i$ are query instances for class $i$, whose distances from each of the class prototypes $\hat{\X}_j$ for all $j \in \mathcal{I}$ are measured in some metric space to determine their class identity. Note that $\Q = \{ \X_i \backslash \hat{\X}_i : i \in \mathcal{I}\}$ is fully specified once we sample $\PP$ from $\pepi(\PP|\Dtr)$. An episode is then defined as a tuple $(\PP,\Q)$.

[]add problem definition]
%\paragraph{Training and Testing} The goal of meta learning based on a metric space is to obtain the optimal embedding function $q_\psi$ for the given series of random splits of $\PP$ and $\Q$. The embedding function $q_\psi$ maps a set to a vector~\cite{snell2017prototypical} or to a distribution~\cite{edwards2016towards}. While using diverse forms of learning objective is possible depending on modeling assumption, for now we simply denote it as a $\loss$. 
%\begin{align}
%\psi^* = \argmin_{\psi} \E_{\pepi(\PP|\Dtr)}\big[ \loss(\psi;\PP,\Q) \big]
%\label{eq:episodic_train}
%\end{align}
%At each stochastic gradient descent step, we approximate the gradient of  \eqref{eq:episodic_train} with a single Monte-Carlo sample $\PP_t$ and $\Q_t$, that is $\grad \loss(\psi;\PP_t,\Q_t)$.
%Testing is done in a similar way. We randomly generate a pre-defined number of episodes (e.g. 1000) from $p_{\text{epi}}(\PP|\Dte)$. For each episode, we calculate accuracy with the learned embedding function $q_{\psi^*}$, and then take the average of theses accuracies.

\subsection{Learning to Generalize to Unseen Classes}
%1. 임베딩 기반 방법은 few-shot learning을 위한 메트릭 공간을 잘 배움  
%2. 그러나 에피소딕 훈련 전략에서, 매 에피소드마다 전체 클래스의 부분 집합인 클래스와 각 클래스들의 데이터를 sampling하고, 해당 에피소드 내에서 분류만 잘 하면 됨. 
%3. higher way란? higher shot이란?
%4. prototypical net은 higher way에서는 잘 되지만 higher shot에는 잘 안 됐음
%5. TPN은 higher shot을 제시했는데.. higher shot은 각 클래스 별로 더 많은 데이터를 보는 셈. 
%6.우리는 메타 트레이닝에서 한 에피소드에서 진행한 클래시피케이션이 다른 샘플링된 클래스를 가진 에피소드의 클래시피케이션에 도움이될 수 있도록 학습을 강제함.
%7. 어떤 모델에도 도움이 될 수 있는 학습 방법 제시. 
In this section, we introduce our novel approach to solve the problem described above. Our goal is to learn embedding space from a set into a distribution in which embedded distributions corresponding to different classes are well separated. % to encode a set into a distribution, which also satisfies discriminativity between classes.
Toward this, we devise a novel loss function $\loss$ that consists of two terms: (i) a generative loss to encode a set into a distribution and (ii) a discriminative loss to locate different distributions in separated regions.

Our generative loss basically is built on similar intuition in   \cite{edwards2016towards}, with slight modification in the graphical structure (see below for details). The original Neural Statistician developed in \cite{edwards2016towards} assumes hierarchical latent variables to generate $\Dtr$: the first variable $\bc$ is to locate class-level variance, and the other variable $\bz$ captures instance-level variance \cite{kingma2014semi}. Each datapoint $\bx$ is assumed to be generated conditionally on those two latent variables. Unlike \cite{edwards2016towards}, we adopt the dependency between variables as shown in Figure \ref{model_gen} to simplify the inference procedure and allow efficient episodic meta-training\footnote{We also used this version of Neural Statistician as our baseline.}. For each episode, the generative process of the sampled dataset $\PP = \{\hat{\X}_1,\dots,\hat{\X}_S\}$ is as follows:
\begin{align}
p(\bc_i) = \N(\mathbf{0}, \bI),\quad p(\bz) = \N(\mathbf{0}, \bI),\quad p(\PP) = \prod_{i \in \mathcal{I}} \int p(\bc_i) \left[ \prod_{\bx \in \hat{\X}_i} \int p(\bz)p_\theta(\bx|\bz,\bc_i) \text{d}\bz \right] \text{d}\bc_i 
\end{align}
where $\theta$ is the collection of parameters for the generative process. Note that the exact posterior of $\bc$ and $\bz$ is intractable. Instead, we resort to variational mean-field approximation with tractable form of lower bound. If we further approximate it with a single Monte-Carlo sample, then we obtain the following generative loss:
\begin{align}
\loss_\text{gen}(\psi,\theta,\phi;\PP) = \sum_{i \in \mathcal{I}} \sum_{\bx \in \hat{\X}_i} \bigg(\log p_\theta(\bx|\tilde{\bc}_i,\tilde{\bz}) - \KL[q_\phi(\bz|\bx)\|p(\bz)]\bigg) - \KL[q_\psi(\bc_i|\hat{\X}_i)\|p(\bc_i)] \label{eq:gen_loss}
\end{align}
where $\tilde{\bc}_i$ and $\tilde{\bz}$ are sampled from $q_\psi(\bc_i|\hat{\X}_i)$ and $q_\phi(\bz|\bx)$ respectively, and backpropagated with reparameterization trick w.r.t. the variational parameters $\psi$ and $\phi$~\cite{kingma2013auto}. 

\begin{figure*}[t]
	\hfill
	\subfigure[generative model]{\includegraphics[height=2.6cm]{figure/model-gen.pdf}\label{model_gen}}
	\hfill
	\subfigure[KL divergence for discriminating between classes]{\includegraphics[height=2.6cm]{figure/loss-disc.pdf}\label{loss_disc}}
	\hfill
	\vspace{-0.1in}
	\caption{\small (a) The generative model for DiVaSE, for each sampled classes $i \in \mathcal{I}$ and dataset $\hat{\X}_i$. The posterior of $\bc_i$ is obtained given a dataset $\hat{\X}_i$, which is the embedding distribution we work with. (b) For all the class pairs $i,j \in \mathcal{I}$, the embedding of each query instance and the that of each support set are compared through KL divergence, to determine class identities of query instances.
	}
	%\vspace{-0.1in}
\end{figure*}

Note that $q_\psi$ is the embedding function discussed above, which maps set $\hat{\X}_i$ to the corresponding posterior distribution of $\bc_i$. In doing so, we use Deep set \cite{zaheer2017deep} to convert the set $\hat{\X}_i$ into a single vector, namely $\bv_i$. Specifically, each elements $\bx \in \hat{\X}_i$ is nonlinearly transformed with multiple layers denoted as $f_\psi(\bx)$ and they are collected and averaged into $\bv_i$. Finally, mean and log variance of $\bc_i$ are generated from $\bv_i$:
\begin{align}
	\bv_i = \frac{1}{\hat{N}_i} \sum_{\bx \in \hat{\X}_i} f_\psi(\bx),\quad q_\psi(\bc_i|\hat{\X}_i) = \N(\bs\mu_\psi(\bv_i),\text{diag}(\bs\sigma_\psi^2(\bv_i)))
\end{align}
In all our experiments, we use a single layer implementation for each $\bs\mu$ and $\bs\sigma$, which seems to perform better than applying additional nonlinearities on $\bv_i$.

%\subsection{Learning to Discriminate between Distributions}
The most critical limitation of \cite{edwards2016towards} as a classifier is that the generative loss $\loss_\text{gen}$ embeds each class set independently. There is no explicit consideration for discriminating between embeddings for different classes, hence they start to collide and the performance degrades even with the moderate number of classes considered at a time. To solve this issue, we propose to minimize the distance $d(\cdot,\cdot)$ between the distribution of prototype set $q_\psi(\bc_i|\hat{\X}_i)$ and that of query instances $q_\psi(\bc_i|\bx), \bx \in (\X_i \backslash \hat{\X}_i)$ if they belong to the same class $i$. Otherwise, we maximize the distance between them:
\begin{equation}
\begin{aligned}
&\loss_\text{disc}(\psi;\PP,\Q) \\
&= \sum_{i \in \mathcal{I}} \left[ \sum_{\bx \in (\X_i \backslash \hat{\X}_i)}d\Big(q_\psi(\bc_i|\hat{\X}_i),q_\psi(\bc_i|\bx)\Big) + \log \sum_{j \in \mathcal{I}} \exp\Big(-d\Big(q_\psi(\bc_i|\hat{\X}_j),q_\psi(\bc_i|\bx)\Big)\Big)\right] \label{eq:disc_loss}
\end{aligned}
\end{equation}
The form of the objective is log of softmax probabilities, which is similar to that of Prototypical Network~\cite{snell2017prototypical}. However, since we need to measure \emph{the similarity between two probabilistic distributions}, Euclidean distance or cosine similarity cannot be used as a proper metric. Here, although it is not a distance, we use Kullback-Leibler (KL) divergence, %such that for some probability distributions $P$ and $Q$,
\begin{align}
d(P,Q) := \KL[P\|Q].
\end{align}
While $\KL$ is not commutative, it turns out using opposite direction of KL divergence still works well mainly because both distributions in \eqref{eq:disc_loss} are in the same Gaussian family. 

%both direction Note that the direction of the divergence is from $Q$ to $P$.

In the episodic training strategy, only subset of classes are sampled (classes in $\mathcal{I}$) and used to construct the discriminative loss in \eqref{eq:disc_loss}. However, we still want to make our embedding function $q_\psi$ to consider even remaining classes (that is, classes not in $\I$) as well, which we call \emph{context classes}: $\C \subset [S]\backslash\I$. In order to achieve this purpose, we propose additional scheme where we periodically (e.g. for every 100th episode) store the set vector $\bv_i$ and use them to maximize the KL divergences even for context classes:    
%the classification within $\I$ also induce the discriminativity within $\C$, as well as between $\I$ and $\C$. Toward this goal, we maximize the KL divergences between the corresponding class pairs.%\footnote{Note that we arbitrarily set the direction of the KL divergence, they and can be changed.}
\begin{align}
\loss_\text{context}(\psi;\PP,\widebar{\mathcal{V}}) = \underbrace{\sum_{i \in \mathcal{I}} \sum_{j \in \mathcal{C}} -d(q_\psi (\bc_i|\hat{\X}_i),q_\psi(\bc_j|\widebar{\bv}_j))}_\text{between sampled and context classes} + \underbrace{\sum_{i \in \mathcal{C}} \sum_{j \in \mathcal{C}} -d(q_\psi (\bc_i|\widebar{\bv}_i),q_\psi(\bc_j|\widebar{\bv}_j))}_\text{within context classes} \label{eq:context_loss}
\end{align}
where we abuse notation and $q_\psi (\bc_i|\widebar{\bv}_i) = \N(\bs\mu_\psi(\widebar{\bv}_i),\text{diag}(\bs\sigma_\psi^2(\widebar{\bv}_i)))$. This scheme is based on past embedding, which is not perfect, but can prevent severe collisions among unselected classes while greatly reducing the computational cost of inferring $q_\psi(\bc_i|\X_i)$ for all classes every episode.

%Here, $\widebar{\bv}_i$ is the set vector stored for each class $i \in [S]$, and we update them periodically with the predefined frequency (e.g. 100). It greatly reduces the computational cost of inferring $q_\psi(\bc_i|\X_i)$ every episode, because we do not have to forward pass $f_\psi(\bx)$ for all $\bx \in \X_i$. In this vein, $q_\psi(\bc_i|\widebar{\bv}_i)$ in \eqref{eq:context_loss} indicates that the posterior of $\bc_i$ can also be inferred from the pre-stored set vector $\widebar{\bv}_i$. The collection of $\widebar{\bv}_i$ for all $i \in [S]$ is denoted as $\widebar{\mathcal{V}}$.
\subsection{Application to Few-shot Learning}
\begin{algorithm}[H]
	\caption{Our alogrithms}\label{algo:divase}
	\begin{algorithmic}[1]
		\State $p(\mathcal{T})$: distribution over tasks
		\State $\alpha, \beta$: step size hyperparameters
		\For{each \emph{epoch}}
		\For{each task $\mathcal{T}_i$ of batch}
		\State Sample K datapoints $\mathcal{D}=\{ x^{(j)}, y^{(j)}\}$ from $\mathcal{T}_i$
		\State Evaluate $\nabla_\theta \mathcal{L}_{Disc}(f_\theta(\mathcal{D}))$ using $\mathcal{D}$ and $\mathcal{L}_{Disc}$ in Equation (1)
		\State Compute adapted parameters with gradient descent:
		\State $\theta'_i \leftarrow \theta - \alpha \nabla_\theta \mathcal{L}_{Disc}(f_\theta)$
		\State Sample datapoints $\mathcal{D}_i'=\{ x^{(j)}, y^{(j)}\}$ from $p(\mathcal{T})$ for the meta-update
		\EndFor
		\State Update $\theta \leftarrow \theta - \beta \nabla_\theta \sum_{\mathcal{T}_i \sim p(\mathcal{T})} \mathcal{L}_{Context}(f_{\theta'}(\mathcal{D}_i'))$ using $\mathcal{L}_{Context}$ in Equation (2)
		\EndFor
	\end{algorithmic}
\end{algorithm}

The final version of our learning algorithm is described in Algorithm \ref{algo:divase}. The model has two hyperparameters $\lambda$ and $\gamma$ for scaling each loss term. We can tune them via cross-validation in practice. More detailed experimental setup is introduced in the next section.


%\begin{algorithm}[H]
%	\caption{Discriminative Variational Set Embedding (DiVaSE) with Contexts}\label{algo:divase}
%	\begin{algorithmic}[1]
%		\For{each \emph{test} episode $t$}
%		\State $\mathcal{I} \leftarrow$ $M$ indices uniformly sampled from $[S]$
%		\State $\mathcal{C} \leftarrow$ $M'$ indices uniformly sampled from $[S]\backslash \mathcal{I}$
%		\Comment{Context classes}
%		\State $\PP, \Q \leftarrow \{ \hat{\X}_i : i \in \mathcal{I} \}, \{\X_i \backslash \hat{\X}_i : i \in \mathcal{I}\}$
%		\Comment{Random split of support and query set}
%		\If{$t$ is at the predefined interval}
%		\State Compute $\widebar{\bv}_i = \frac{1}{\hat{N}_i} \sum_{\bx \in \hat{\X}_i} f_\psi(\bx),\quad \forall i \in [S]$
%		\State $\widebar{\mathcal{V}} \leftarrow (\bv_1,\dots,\bv_S)$
%		\Comment{Update set vectors and store them}
%		\EndIf
		
%		\State $\loss_t \leftarrow \loss_\text{gen}(\psi, \theta, \phi;\PP) + \lambda \loss_\text{disc}(\psi;\PP,\Q) + \gamma \loss_\text{context}(\psi;\PP,\widebar{\mathcal{V}})$
%		\State Update parameters with $\grad\loss_t$
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}

%\begin{figure*}[t]
%	\centering
%	\includegraphics[height=3.2cm]{figure/loss_context.pdf}\label{loss_context}
%	\vspace{-0.1in}
%	\caption{\small dsdd
%	}
%	\vspace{-0.1in}
%\end{figure*}

==> experiments_backup.tex <==
\section{Experiment}

\paragraph{Datasets} We validate our framework on two benchmark datasets for few-shot classification.

\textbf{1) \textit{mini}-ImageNet.} This dataset is a subset of a ImageNet~\cite{krizhevsky2012imagenet} which consists of 100 classes with 600 examples. We followed the dataset split and pre-processing procudure described in ~\cite{ravi2016optimization}, which divides the dataset into 64/16/20 classes for training/validation/test, and resizes original image into $84 \times 84$ pixels.

\textbf{2) \textit{tiered}-ImageNet.} This dataset is also a subset of the ImageNet~\cite{krizhevsky2010convolutional} with 608 classes. We split the dataset into 351/97/160 classes for train/validation/test set and followed other experiment settings as described in ~\cite{ren2018meta}.

\paragraph{Implementation Details}
We adopt the same network architectures that were used for baselines for fair comparison. The base networks of Prototypical Network and Relation Net~\cite{snell2017prototypical, yang2018learning} have 4 layers of convolutional blocks where each block contains 64 filters, $3 \times 3$ convolution layer, a batch normalization, a ReLU activation function and $2\times 2$ max pooling layer at the end of each block. L2G + RN adopts the network architecture of Relation Net which consists of four convolutional blocks as an embedding function and two convolutional blocks and two fully connected layers for the relation module. 

We use Adam optimizer~\cite{kingma2014adam} for all the experiments. We set the learning rate $\alpha$ to 0.001, the number of tasks for the backward propagation to 5 and the initial learning rate to $10^{-3}$ which is multiplied by $0.5$ at every 10K episode for L2G + Proto and 100K episodes for L2G + RN.

\subsection{$N$-way $K$-shot Classification}
\input{mimgnet_table}
\input{timgnet_table}

We evaluate our Learning to Generalize framework first on the conventional $N$-way $K$-shot classification task against relevant baselines~\cite{maml, snell2017prototypical, yang2018learning}. Following ~\cite{snell2017prototypical}, we trained and evaluated models over large number of episodes, which randomly sample $N$ classes with $K$ support and $M$ query examples at each task. For our Learning to Generalize framework, we generate and sample two episodes at each iteration in meta-training time, for task-specific learning and generalization. Note that the episode used for inner loop does not participate in the outer loop classification, which is clearly different from the "higher way" or "higher shot" setttings described in ~\cite{snell2017prototypical} where more sampled classes or examples also participate in the classification. At meta-test time, our model classifies between the given unseen classes with the initial model without any further training.

%also use a single episode at each iteration, and we provide evaluation performance attained from the inner loop for fair comparison.

% 15-query 넣어야함.
We provide few-shot classification result under 5 and 10-way settings of \textit{mini}-ImageNet in Table~\ref{tbl:mini} and \textit{tiered}-ImageNet in Table~\ref{tbl:tiered} respectively. The results clearly show the effectiveness of L2G framework, since both models trained with our meta-learning framework outprforms the baselines across all conditions. Specifically, when it comes to 1-shot classification, which has insufficient information for the inference, the L2G framework yields even larger performance improvements, with at most 4.89\% gain for 5-way 1-shot on \textit{tiered}-ImageNet over the baseline. 

\input{visualization}
\input{loss_plot}
We further provide the learned embedding visualization of the models in Figure~\ref{fig:vis}, which confirms the effectiveness of our bilevel optimization framework. Compared with the original Prototypical Networks model, the model with L2G shows clean separation between classes. The L2G+Prototypical Networks, at meta-test phase, provides much smaller and well-clustered embeddings for the unseen classes. The convergence plot in Figure~\ref{fig:convergence} provides episodic training loss at meta-training stage. While our model converges slightly slowly compared to the base model, it eventually converges at lower loss. 


\subsection{\textit{Any}-way \& \textit{Any}-shot Classification}

To validate the leverage of generic information transfer, we introduce a novel \textit{any}-way \textit{any}-shot classification task, where both the number of shots and classes in each episode can largely vary. Table~\ref{tbl:mini-any} shows the results of the base model and ours on the \textit{mini}-ImageNet dataset. For any-shot classification, the number of shot randomly varies between ${1,5,10}$-shots for each episode, and simliarly, the number of classes at each episode randomly varies between ${5,7,10}$-ways for any-way setting. Then, we fix the first task to a 5-shot classification problem and the generalization task to contain any-shot any-way classification problems. The number of queries and ways for both tasks is fixed as 15, 5, respectively. In the same manner, we train the Prototypical Network with randomly sampled shot among 1, 5, 10 for each episode. For any-way classification tasks, the number of classes is given among 5, 7, 10. Similarly to any-shot classification, we fix the first tasks as a 5-way 5-shot classification task and check whether the model trained with small tasks can generalize to classification tasks with various numbers of unseen classes and instances. We sample classes disjointly for the first and the second task. For Prototypical Networks, we randomly change the number of way between 5, 7, 10. In meta-test phase, we iteratively change the number of shot and way as ${1, 5, 10}$ and ${5, 7, 10}$, respectively with 600 episodes. In the case of any-shot \& any-way classification, we vary both shots and ways. 
\input{anyshotway_table}
Table~\ref{tbl:mini-any} shows the results. We observe that combining L2G framework with the model consistantly improves over the base model, suggesting that it learned to generalize to unseen tasks with varying number of classes and instances. Note that our model have 1.98 \% higher accuracy than the baseline for \textit{Any}-shot \& \textit{Any}-way tasks which are most difficult, as they require to generalize to unseen tasks.


==> implementation_detail.tex <==
\paragraph{Implementation Details}
In all experiments, models use Adam~\cite{kingma2014adam} with initial learning rate 1e-3, and annealed by half every 10,000 episodes. For Omniglot and Omniglot+MNIST datasets, the meta-learner uses a shallow neural network with three fully connected layers. The dimension of a c layer and a z layer is 32 units for distribution estimators, and 64 units single c layer for point estimators. For AwA, a neural network with 4 convolutional blocks introduced in ~\cite{vinyals2016matching} is used. Each block contains convolution layer with 3x3 convolution, 64 filters, and followed by batch normalization, ReLU and 2x2 max pooling layer. For distribution estimators, 128 and 64 units are used for c and z layers, and 192 units are used for c layer with point estimators. We attached classifier with softmax for the CNN to properly learn high level concept. All the experiments are repeated for 5 times and reported averaged performance. For each of the results reported is averaged over 1000 episodes for N-way K-shot test and 20 episodes for Full-way K-shot test with 95\% confidence intervals.

==> incremental.tex <==
\subsubsection{Incremental Learning}
Any-shot learning is closely related to incremental learning. When we measure performance at each test episode $t \in [T]$, in incremental learning framework, it is allowed to use and incorporate the test results at time $t-1$. When $t$ is very small such that we just started testing, then the number of support instances for each class would be only one or a few, which corresponds to conventional one/few-shot learning. As the testing proceeds, the number of instances for each class rapidly grows as we incorporate more instances, and the problem becomes many-shot learning. Thus, the effective number of shot is \emph{any}. %Also, it is crucial to \emph{rapidly} incorporate the knowledge into the model, such that the whole testing time is manageable. 
Set encoding is an efficient solution for this problem. Algorithm \ref{algo:incremental} shows each step of the incrementally learning framework.
\begin{algorithm}[H]
	\caption{Any-shot Learning for Incremental Learning}\label{algo:incremental}
	\begin{algorithmic}[1]
		\State $q_\psi \leftarrow$ \Call{AnyShotLearning}{$\D$} \Comment{$\D$ may or may not be imbalanced}
		\State $\mathcal{S}\leftarrow$ \Call{SampleOneWithoutReplacement}{$\D'$}	
		%\State Randomly Sample $\hat{\bx}_i \in X_i$, then $X_i \leftarrow X_i \backslash \{\hat{\bx}_i\}$ for each class $i \in \{S+1,\dots,S+U\}$
		%\State Initialize $\mathcal{S} \leftarrow \{\hat{\bx}_{S+1},\dots,\hat{\bx}_{S+U}\}$
		\Comment{Support set}
		\While{$\D' \neq \emptyset$}
%		%\State Sample $\hat{N}_{S+1},\dots,\hat{N}_{S+U} \sim \pepi(\hat{N}_{S+1},\dots,\hat{N}_{S+U})$
%		\For{each \emph{test} class $i \in \{S+1,\dots,S+U\}$}
		%\State Uniformly Sample $\hat{\bx}_i \in X_i$
		%\State $X_i \leftarrow X_i \backslash \{\hat{\bx}_i\}$
		%\EndFor
		\State $\mathcal{Q}\leftarrow$ \Call{SampleOneWithoutReplacement}{$\D'$}
		\Comment{Query set}
		%\State $\hat{\D}_t \leftarrow \hat{\D}_{t-1} \cup \{ \hat{\bx}_{S+1},\dots,\hat{\bx}_{S+U} \}$
		\State Calculate accuracy with each element in $\mathcal{S}$ and $\mathcal{Q}$ embedded with $q_\psi$.
		\State $\mathcal{S} \leftarrow \mathcal{S} \cup \mathcal{Q}$
		\Comment {Support set $\mathcal{S}$ is gradually expanding }
		\EndWhile
	\end{algorithmic}
\end{algorithm}

==> intro_backup.tex <==
\section{Introduction}
While deep learning models such as CNNs have been proven effective on multi-class classification~\citet{alexnet,resnet,densenet}, even surpassing human performances~\citet{imagenet}, such impressive performances are obtained with the availability of large number of training instances per class. However, in more realistic settings where we could have very few training instances for some classes, deep learning models may fail to obtain good accuracies due to overfitting. On the other hands, humans can generalize surprisingly well even with a single instance from each class. This problem, known as the few (one)-shot learning problem, thus has recently attracted large attention, leading to the proposal of many prior work that aim to prevent the model from overfitting when trained with few instances.

Recently, meta-learning approaches that learn to generalize over multiple tasks (learning to learn)~\citet{vinyals2016matching,santoro2016meta,rezende2016one,snell2017prototypical} have obtained impressive performances on the few-shot learning tasks. They tackle the low-data challenge in few-shot learning by learning a classifier to solve any few-shot learning problem well, by training over large number of episodes, where in each episode the model randomly solves a different few-shot classification problem. A popular approach in composing such meta knowledge is to assume some common metric space and learn the optimal embedding function on it. Matching Networks~\citet{vinyals2016matching} and Prototypical Networks~\citet{snell2017prototypical} are examples of such embedding approaches, which are known to perform well and computationally efficient as well. 

However, these approaches are limited in that they assume for each episode, the prototype set of each class is sampled and \emph{mapped into a single point} in the metric space (e.g. embedding mean). Then the distance (e.g. Euclidean) between class prototypes and query instances are measured to determine their class identities, without consideration of other statistics of the sets such as variance. This point estimation of the true population 
%can easily overfit and poorly generalize on unseen classes, due to the 
suffers from lack of robustness in its estimation,
%. Such a crude estimation 
%which limits its applicability to more realistic settings.
which limits its generalization ability to unseen classes.

%First, point estimation cannot represent the variance w.r.t. the number of elements in the set. If the set consists of only a single element, then the uncertainty should increase, as we estimate the whole class population with this single sample. However, point estimation will simply embed the only available sample as a prototype for the class, which is problematic if this sample is highly biased. In this case, variance needs to be learned to cover other instances from the same class (See Figure~\ref{fig:1shot}). Moreover, considering that real-world datasets may be highly imbalanced in the number of instances per class, the ability of learning different amount of uncertainties for each class is crucial.
Specifically, when we have a biased sample and want it to represent the true class population, the uncertainty should increase to make the prototype to cover other instances from the same class population (See Figure~\ref{fig:concept1}). However, point estimation cannot represent uncertainty as it only consider the sample mean and no other statistics. Therefore, whenever we sample such biased examples as a class prototype, point estimation is likely to propagate wrong information without letting query instances be aware of the risks, resulting in degraded performance in the classification. It can be prevented by learning proper amount of uncertainties for each sampled prototype set.

\begin{figure*}[t]
	\hfill
	\subfigure[]{\includegraphics[height=3.7cm]{figure/concept2.pdf}\label{fig:concept1}}
	\hfill
	\subfigure[]{\includegraphics[height=3.7cm]{figure/concept1.pdf}\label{fig:concept2}}
	\hfill
	\subfigure[]{\includegraphics[height=3.7cm]{figure/concept3.pdf}\label{fig:concept3}}
	\hfill
	\vspace{-0.1in}
	\caption{\small \textbf{Concepts.} (a) When the outlier sample locates far from the true population, it is very risky to use this sample as the class prototype. However, the problem is much alleviated with large variance to cover the true population. (b) Variance with respect to the different level of diversity of set elements.  (c) In point estimation, equal distance metric is applied along all directions, and it is hard to know which direction is more sensitive (or important) than the other in classfication. On the other hand, if the class instances are more likely to locate along some specific dimensions (y-axis in the example) and in a similar vein learned variances also have narrow shapes along those dimensions, then different distance metrics can be applied along each dimension, such that some dimension (x-axis in the example) has more sensitive distance metric than the other. }
	\vspace{-0.2in}
\end{figure*}

%\begin{wrapfigure}{r}{0.3\textwidth}
%	\vspace{-0.15in}
%	\centering
%	\includegraphics[width=1.0\linewidth]{figure/concept_set.png}
%	\vspace{-0.25in}
%	\caption{\textbf{Learned Variances from DiVaSE.} The learned variance from the set with high diversity (red) is larger than the variance from the set with low diversity (green).}
%	\vspace{-0.1in}
%	\label{concept}
%\end{wrapfigure}

Another limitation of point estimate is that it cannot represent the diversity among the elements in the prototype set. Even with the same number of samples for each episode (or shots), the sets may have varying degree of diversity (See Figure \ref{fig:concept2}). However, point estimation of the class embedding cannot yield any more informative statistics than their mean, and thus cannot fully exploit the benefit of having multiple samples to represent a class.

Finally, the sets representing classes should be discriminatively embedded, but with a point estimate of the class embedding it is not clear if the two sets are well separated unless there exists additional samples from the two classes that can be used to generate discriminative constraints (an instance should be closer to its own class prototype than other class prototypes). Constraining the embeddings to have minimum distances among them is one solution but it does not consider which dimension is more important than others when discriminating between the two (See Figure \ref{fig:concept3}). In fine-grained classification problems, two classes may be very similar in all features but one. 

In conclusion, we need to develop a method that can well represent a given set, such that sets with 
%smaller number of instances or with high diversity
biased samples or high variance
should be mapped to a distribution with larger variance, to more accurately reflect uncertainty 
%and variance 
in the true population. In this sense, \emph{representing each class prototype set as a distribution} is a very natural way to improve upon the current point-estimate based few-shot learning approaches. Such a probabilistic embedding model will be more robust to overfitting and 
%can be applied to more realistic settings.
generalize better on unseen classes.

Lastly, 
%a secondary
another important
advantage of a set embedding method is that all the sampled instances can be set-wisely embedded at once, leading to less computational complexity compared to embedding all individual elements. For example, when we perform classification given a handful of prototype sets and query instances for each episode, we can make this classification loss to induce that the other classes that do not participate in the classification also discriminate each other, in a \emph{set-wise manner} (See Figure {\color{red}2}). Exploiting such computational efficiency, we explicitly train the meta-learner to improve the generalization performance on unseen classes in the meta-test dataset. Note that simply increasing the number of classes (or way) at training time is expensive because the number of pairs of a prototype and a query instance increases quadratically. We can minimize the compuational cost by encapsulating the whole set into a single distribution, and efficiently performing set-wise discrimination.

We validate our model on multiple public benchmark datasets for few-shot classification task against state-of-the-art few-shot meta-learning models, of which our model significantly outperforms.

In summary, our contribution is twofold:

\begin{itemize}
%\item We tackle the problem of \emph{any-shot learning} which is a more realistic setting for classification where each class can come with any number of instances, to bridge the gap between conventional many-shot learning and few-shot learning. 
\item We propose a novel \emph{discriminative variational set embedding} (DiVaSE) model that discriminatively embeds an entire set into a Gaussian distribution, whose mean and variance is learned with variationl inference to consider both the uncertainty and diversity among the embedded samples, as well as to maximize discriminativity among classes.  
\item Using our discriminative variational set embedding model, we propose an efficient meta-learning algorithm that explicitly targets to improve generalization to unseen classes, by introducing a contextual loss for performing set-wise discrimiation between meta-test classes.
%\item We propose a \emph{meta-learning} algorithm for any-shot learning that trains the model with various sets with different size and class labels, that can robustly tackle the problem of anyshot learning and also generalizes well to unseen classes.
\end{itemize}



==> main_table.tex <==
\begin{table}[!htbp]
	\centering
	\small
	\begin{tabular}{c c c c c c}
		$M$-Way & $K$-Shot & DPSE & N. Stat & RN & Proto\\
		\midrule
		\midrule
		\multirow{2}{*}{5} & 1  & $ \textbf{91.12} \pm \textbf{0.23} $ & $ 54.42 \pm 1.62 $ & $ 86.89 \pm 1.70 $ & $ 87.38 \pm 0.38 $ \\ \cmidrule(l){2-6}
		& 5  & $ \textbf{97.20} \pm \textbf{0.26} $ & $ 84.99 \pm 035 $ & $ 95.63 \pm 0.31 $ & $ 96.87 \pm 0.09 $ \\ % \cmidrule(l){2-6}
		%& Any-shot & 1-shot & $ \textbf{92.00} \pm \textbf{0.33} $ & $ 67.01 \pm 1.50 $ & $ 87.31 \pm 0.31 $ & $ 91.00 \pm 0.18 $ \\ \cmidrule(l){2-6}
		%& Any-shot & 5-shot & $ 97.43 \pm 0.60 $ & $ 79.19 \pm 2.18 $ & $ 94.22 \pm 0.49 $ & $ 97.04 \pm 0.11 $ \\ \cmidrule(l){2-6}
		%& Any-shot & Any-shot & $ 94.96 \pm 0.28 $ & $ 73.55 \pm 1.78 $ & $ 91.33 \pm 0.52 $ & $ 94.29 \pm 0.18 $ \\
		
		\midrule
		\midrule
		\multirow{2}{*}{Full} & 1  & $ \textbf{22.24} \pm \textbf{0.03} $ & $ 6.29 \pm 0.92 $ & $ 12.62 \pm 1.69 $ & $ 17.44 \pm 0.22 $ \\ \cmidrule(l){2-6}
		& 5  & $ \textbf{44.60} \pm \textbf{0.36} $ & $ 14.59 \pm 1.29 $ & $ 30.29 \pm 0.16 $ & $ 41.53 \pm 0.47 $ \\ %\cmidrule(l){2-6}
		%& Any-shot & 1-shot & $  \pm  $ & $  \pm  $ & $  \pm  $ & $ 21.25 \pm 0.21 $ \\ \cmidrule(l){2-6}
		%& Any-shot & 5-shot & $  \pm  $ & $  \pm  $ & $  \pm  $ & $ 40.45 \pm 0.34 $ \\ %\cmidrule(l){2-6}
		%& Any-shot & Any-shot & $  \pm  $ & $  \pm  $ & $  \pm  $ & $ 31.33 \pm 0.25 $ \\
		\midrule
		\midrule
	\end{tabular}\caption{\small Generalization performance on Omniglot}\label{omniglot-table}
\end{table}

\begin{table}[!htbp]
	\centering
	\small
	\begin{tabular}{c c c c c c}
		$M$-Way & $K$-Shot & DPSE & N. Stat & RN & Proto\\
		\midrule
		\midrule
		\multirow{1}{*}{5} %& 1 / 1 & $ \textbf{50.36} \pm \textbf{1.21} $ & $ 45.33 \pm 1.81 $ & $ 45.96 \pm 1.65 $ & $ \textbf{49.95} \pm \textbf{0.98} $ \\ \cmidrule(l){2-6}
				   %& 5 / 5 & $ \textbf{70.37} \pm \textbf{1.75} $ & $ \textbf{69.31} \pm \textbf{1.04} $ & $ 58.85 \pm 1.64 $ & $ 67.86 \pm 1.33 $ \\ \cmidrule(l){2-6}
				   %& Any / 1 & $ \textbf{50.20} \pm \textbf{0.64} $ & $ \textbf{51.25} \pm \textbf{0.61} $ & $ 46.54 \pm 0.89 $ & $ 50.55 \pm 0.77 $ \\ \cmidrule(l){2-6}
				   %& Any / 5 & $ \textbf{68.97} \pm \textbf{1.14} $ & $ 67.54 \pm 1.02 $ & $ 58.72 \pm 1.18 $ & $ 66.51 \pm 1.03 $ \\ \cmidrule(l){2-6}
				   & Any / Any & \bf65.60 $\pm$ 0.77 & 65.06 $\pm$ 1.08 & $ 57.11 \pm 1.03 $ & $ 63.60 \pm 0.87 $ \\
				   
		\midrule
		\midrule
		\multirow{1}{*}{Full} %& 1 / 1 & $ \textbf{16.90} \pm \textbf{0.42} $ & $ \textbf{16.54} \pm \textbf{1.09} $ & $ 10.39 \pm 1.36 $ & $ 14.84 \pm 0.30 $ \\ \cmidrule(l){2-6}
							%& 5 / 5 & $ \textbf{33.08} \pm \textbf{1.40} $ & $ 27.98 \pm 1.88 $ & $ 19.14 \pm 2.60 $ & $ 27.22 \pm 0.60 $ \\ \cmidrule(l){2-6}
							%& Any / 1 & $ \textbf{17.79} \pm \textbf{0.71} $ & $ 16.05 \pm 0.54 $ & $ 11.62 \pm 1.39 $ & $ 14.35 \pm 0.30 $ \\ \cmidrule(l){2-6}
							%& Any / 5 & $ \textbf{30.74} \pm \textbf{1.59} $ & $ 26.96 \pm 1.30 $ & $ 11.85 \pm 2.35 $ & $ 25.24 \pm 0.50 $ \\ \cmidrule(l){2-6}
							& Any / Any & $ \textbf{30.25} \pm \textbf{1.48} $ & $ 26.10 \pm 1.23 $ & $ 17.16 \pm 2.48 $ & $ 23.55 \pm 0.39 $ \\
		\midrule
		\midrule
	\end{tabular}\caption{\small Generalization performance on Omniglot+MNIST imbalanced dataset}\label{omnist-table}
\end{table}

\begin{table}[!htbp]
	\centering
	\small
	\begin{tabular}{c c c c c c}
		$M$-Way & $K$-Shot & DPSE & N. Stat & RN & Proto\\
		\midrule
		\midrule
		\multirow{5}{*}{5} & 1 / 1 & $ 40.04 \pm 1.42 $ & $  \pm  $ & $ xx.xx \pm xx.xx $ & $ \textbf{40.55} \pm \textbf{0.39} $ \\ \cmidrule(l){2-6}
							& 5 / 5 & $ \textbf{70.67} \pm \textbf{1.48} $ & $ 62.03 \pm 0.87 $ & $  \pm  $ & $ \textbf{69.64} \pm \textbf{0.10} $ \\ \cmidrule(l){2-6}
							& Any / 1 & $ \textbf{44.06} \pm \textbf{0.56} $ & $ 41.28 \pm 0.85 $ & $  \pm  $ & $ 43.41 \pm 1.05 $ \\ \cmidrule(l){2-6}
							& Any / 5 & $ \textbf{67.86} \pm \textbf{0.29} $ & $ 62.96 \pm 0.79 $ & $  \pm  $ & $ 67.19 \pm 1.15 $ \\ \cmidrule(l){2-6}
							& Any / Any & $ \textbf{79.23} \pm \textbf{0.71} $ & $ 76.03 \pm 1.14 $ & $ \pm  $ & $ \textbf{78.62} \pm \textbf{1.00} $ \\
		
		\midrule
		\midrule
		\multirow{5}{*}{Full} & 1 / 1 & $ \textbf{26.03} \pm \textbf{1.99} $ & $  \pm  $ & $  \pm  $ & $ 25.08 \pm 0.75 $ \\ \cmidrule(l){2-6}
								& 5 / 5 & $ \textbf{55.03} \pm \textbf{2.13} $ & $ 43.43 \pm 3.01 $ & $  \pm  $ & $ 52.27 \pm 0.84 $ \\ \cmidrule(l){2-6}
								& Any / 1 & $ 27.66 \pm 1.38 $ & $ 26.70 \pm 0.76 $ & $  \pm  $ & $ \textbf{29.55} \pm \textbf{0.67} $ \\ \cmidrule(l){2-6}
								& Any / 5 & $ \textbf{52.77} \pm \textbf{0.78} $ & $ 46.75 \pm 2.99 $ & $  \pm  $ & $ 50.72 \pm 2.40 $ \\ \cmidrule(l){2-6}
								& Any / Any & $ \textbf{65.34} \pm \textbf{2.26} $ & $ 61.39 \pm 3.50 $ & $  \pm  $ & $ \textbf{65.79} \pm \textbf{2.04} $ \\
		\midrule
		\midrule
	\end{tabular}\caption{\small Generalization performance on AwA}\label{awa-table}
\end{table}

==> omni_table.tex <==
\begin{table}[t]
	\small
	\caption{Omniglot few-shot classification.} 
	\begin{center}
		\begin{tabular}{ccccc}
		\hline
		& \multicolumn{1}{c}{20-way} & \multicolumn{1}{c}{30-way} & \multicolumn{1}{c}{40-way} & \multicolumn{1}{c}{50-way} \\\cmidrule{2-5}
			Models & 1-shot & 1-shot & 1-shot & 1-shot  \\
			\hline
			\hline
			Prototypical Network & 96.0 & 95.56 & 94.80 & 94.26  \\ 
			L2G + Proto &  97.24 & 95.92  &94.87 & 94.03 \\
			\hline
			Relation Network &  97.6 & 96.11  & 95.34  &  94.62 \\
			L2G + RN &  97.56 & 95.49  & 94.61 &  93.91 \\
			\hline
			
		\end{tabular}\label{tbl:omni}
		\vspace{-0.15in}
	\end{center}
\end{table}

